Resilient Urban Housing Markets: Shocks vs. Fundamentals

In the face of a pandemic, urban protests, and an affordability crisis, is the desirability of dense urban settings at a turning point? Assessing cities' long term trends remains challenging. The first part of this chapter describes the short-run dynamics of the housing market in 2020. Evidence from prices and price-to-rent ratios suggests expectations of resilience. Zip-level evidence suggests a short-run trend towards suburbanization, and some impacts of urban protests on house prices. The second part of the chapter analyzes the long-run dynamics of urban growth between 1970 and 2010. It analyzes what, in such urban growth, is explained by short-run shocks as opposed to fundamentals such as education, industrial specialization, industrial diversification, urban segregation, and housing supply elasticity. This chapter's original results as well as a large established body of literature suggest that fundamentals are the key drivers of growth. The chapter illustrates this finding with two case studies: the New York City housing market after September 11, 2001; and the San Francisco Bay Area in the aftermath of the 1989 Loma Prieta earthquake. Both areas rebounded strongly after these shocks, suggesting the resilience of the urban metropolis.

==> tables/city_dynamics_long_run.tex <==

\begin{tabular}{l c c c c c c c c c c c}
\hline
 & Model 1 & Model 2 & Model 3 & Model 4 & Model 5 & Model 6 & Model 7 & Model 8 & Model 9 & Model 10 & Model 11 \\
\hline
(Intercept)                                     & $29.04^{**}$  & $-18.83^{**}$  & $15.41^{***}$  & $-260.28^{***}$ & $5.54$         & $-9.07^{**}$  & $-9.07^{**}$  & $0.00$   & $0.01$   & $0.09$    & $-204.89^{*}$  \\
                                                & $(10.80)$     & $(6.09)$       & $(4.12)$       & $(62.11)$       & $(4.34)$       & $(3.22)$      & $(3.22)$      & $(2.35)$ & $(2.34)$ & $(2.39)$  & $(86.50)$      \\
dissimilarity\_black\_pop                       & $-44.41^{**}$ &                &                &                 &                &               &               &          &          &           & $-47.15^{**}$  \\
                                                & $(15.89)$     &                &                &                 &                &               &               &          &          &           & $(17.35)$      \\
missing\_dissimilarityTRUE                      & $-1.24$       &                &                &                 &                &               &               &          &          &           & $20.82$        \\
                                                & $(20.95)$     &                &                &                 &                &               &               &          &          &           & $(20.90)$      \\
frac\_college\_grads                            &               & $175.58^{***}$ &                &                 &                &               &               &          &          &           & $87.64$        \\
                                                &               & $(52.66)$      &                &                 &                &               &               &          &          &           & $(64.11)$      \\
elasticity                                      &               &                & $9.79$         &                 &                &               &               &          &          &           & $9.36^{*}$     \\
                                                &               &                & $(5.33)$       &                 &                &               &               &          &          &           & $(4.58)$       \\
missing\_elasticityTRUE                         &               &                & $-21.90^{***}$ &                 &                &               &               &          &          &           & $-21.69^{***}$ \\
                                                &               &                & $(4.92)$       &                 &                &               &               &          &          &           & $(5.58)$       \\
share\_agriculture                              &               &                &                & $13.62^{**}$    &                &               &               &          &          &           & $14.76^{*}$    \\
                                                &               &                &                & $(4.94)$        &                &               &               &          &          &           & $(6.37)$       \\
share\_metal\_mining\_oil                       &               &                &                & $0.06$          &                &               &               &          &          &           & $0.12$         \\
                                                &               &                &                & $(0.25)$        &                &               &               &          &          &           & $(0.27)$       \\
share\_construction                             &               &                &                & $8.45^{***}$    &                &               &               &          &          &           & $5.44^{**}$    \\
                                                &               &                &                & $(1.53)$        &                &               &               &          &          &           & $(2.09)$       \\
share\_manufacturing                            &               &                &                & $0.33$          &                &               &               &          &          &           & $-0.91$        \\
                                                &               &                &                & $(1.19)$        &                &               &               &          &          &           & $(1.80)$       \\
share\_transportation\_utilities                &               &                &                & $1.22$          &                &               &               &          &          &           & $1.58$         \\
                                                &               &                &                & $(2.45)$        &                &               &               &          &          &           & $(3.19)$       \\
share\_finance\_ins\_re                         &               &                &                & $6.42^{**}$     &                &               &               &          &          &           & $3.71$         \\
                                                &               &                &                & $(2.11)$        &                &               &               &          &          &           & $(2.59)$       \\
share\_non\_classifiable                        &               &                &                & $8.52^{***}$    &                &               &               &          &          &           & $5.18^{*}$     \\
                                                &               &                &                & $(1.69)$        &                &               &               &          &          &           & $(2.38)$       \\
share\_retail                                   &               &                &                & $1.33$          &                &               &               &          &          &           & $3.30^{*}$     \\
                                                &               &                &                & $(1.02)$        &                &               &               &          &          &           & $(1.41)$       \\
hhi\_q(2.31e+03,2.39e+03]                       &               &                &                &                 & $-5.95$        &               &               &          &          &           & $-4.70$        \\
                                                &               &                &                &                 & $(6.31)$       &               &               &          &          &           & $(6.30)$       \\
hhi\_q(2.39e+03,2.51e+03]                       &               &                &                &                 & $-12.02^{*}$   &               &               &          &          &           & $-6.26$        \\
                                                &               &                &                &                 & $(6.08)$       &               &               &          &          &           & $(7.56)$       \\
hhi\_q(2.51e+03,1.29e+04]                       &               &                &                &                 & $-42.33^{***}$ &               &               &          &          &           & $-34.25^{**}$  \\
                                                &               &                &                &                 & $(8.36)$       &               &               &          &          &           & $(11.82)$      \\
one\_or\_more\_riot\_with\_damage\_propertyTRUE &               &                &                &                 &                & $-2.54$       & $-9.40$       &          &          &           & $-9.60$        \\
                                                &               &                &                &                 &                & $(7.02)$      & $(10.43)$     &          &          &           & $(6.67)$       \\
na\_riot\_with\_damage\_propertyTRUE            &               &                &                &                 &                & $23.97^{***}$ & $23.97^{***}$ &          &          &           &                \\
                                                &               &                &                &                 &                & $(4.80)$      & $(4.80)$      &          &          &           &                \\
total\_riot\_with\_damage\_property             &               &                &                &                 &                &               & $4.18$        &          &          &           &                \\
                                                &               &                &                &                 &                &               & $(4.70)$      &          &          &           &                \\
nbr\_events                                     &               &                &                &                 &                &               &               & $-0.02$  &          &           &                \\
                                                &               &                &                &                 &                &               &               & $(2.69)$ &          &           &                \\
total\_property\_damages                        &               &                &                &                 &                &               &               &          & $-0.02$  &           &                \\
                                                &               &                &                &                 &                &               &               &          & $(0.81)$ &           &                \\
any\_eventTRUE                                  &               &                &                &                 &                &               &               &          &          & $-1.89$   & $2.48$         \\
                                                &               &                &                &                 &                &               &               &          &          & $(10.79)$ & $(10.37)$      \\
\hline
R$^2$                                           & $0.03$        & $0.04$         & $0.07$         & $0.29$          & $0.10$         & $0.09$        & $0.09$        & $0.00$   & $0.00$   & $0.00$    & $0.35$         \\
Adj. R$^2$                                      & $0.03$        & $0.03$         & $0.06$         & $0.27$          & $0.09$         & $0.08$        & $0.08$        & $-0.00$  & $-0.00$  & $-0.00$   & $0.30$         \\
Num. obs.                                       & $306$         & $306$          & $306$          & $306$           & $251$          & $306$         & $306$         & $306$    & $306$    & $306$     & $251$          \\
\hline
\multicolumn{12}{l}{\scriptsize{$^{***}p<0.001$; $^{**}p<0.01$; $^{*}p<0.05$}}
\end{tabular}



==> tables/current_suburbanization_distance.tex <==

\begin{tabular}{l c c c}
  \toprule
 & \multicolumn{3}{c}{Dependent variable: YoY Price Appreciation} \\
  \cmidrule(lr){2-4}
Time period: & 2015--2019 & March-July 2019 & March-July 2020 \\
\midrule
(Intercept)          & $-0.750^{***}$ & $1.067^{***}$ & $-0.806^{***}$ \\
                     & $(0.102)$      & $(0.204)$     & $(0.211)$      \\
Distance to center (km) & $-0.004^{***}$ & $-0.007$      & $0.023^{***}$  \\
& $(0.001)$      & $(0.005)$     & $(0.006)$      \\
Additional controls & \multicolumn{3}{c}{Year fixed effects} \\
\midrule
R$^2$                & $0.013$        & $0.003$       & $0.024$        \\
Adj. R$^2$           & $0.013$        & $0.001$       & $0.022$        \\
Num. obs.            & $13439$        & $581$         & $541$          \\
\bottomrule
\multicolumn{4}{l}{\scriptsize{$^{***}p<0.01$; $^{**}p<0.05$; $^{*}p<0.1$}}
\end{tabular}



==> tables/sf1989_earthquake_fundamentals.tex <==

\begin{tabular}{l c c c}
\hline
 & Model 1 & Model 2 & Model 3 \\
\hline
share\_liquefaction     & $-43.05^{*}$ & $-24.45$  & $-15.42$  \\
                        & $(19.91)$    & $(18.41)$ & $(25.83)$ \\
\hline
Num. obs.               & $1791$       & $1791$    & $1791$    \\
R$^2$ (full model)      & $0.15$       & $0.03$    & $0.02$    \\
R$^2$ (proj model)      & $0.00$       & $0.00$    & $0.00$    \\
Adj. R$^2$ (full model) & $0.15$       & $0.03$    & $0.01$    \\
Adj. R$^2$ (proj model) & $-0.00$      & $-0.01$   & $-0.01$   \\
Num. groups: COUNTYFP10 & $12$         & $12$      & $12$      \\
\hline
\multicolumn{4}{l}{\scriptsize{$^{***}p<0.001$; $^{**}p<0.01$; $^{*}p<0.05$}}
\end{tabular}



==> tables/sf1989_earthquake_pop_change.tex <==

\begin{tabular}{l c c c}
\hline
 & $\Delta$ log(Pop) 1990--1980 & $\Delta$ log(Pop) 2000--1990 & $\Delta$ log(Pop) 2010--2000 \\
\hline
(Intercept)         & $0.29^{***}$ & $0.16^{***}$ & $0.10^{***}$ \\
                    & $(0.02)$     & $(0.01)$     & $(0.02)$     \\
share\_liquefaction & $-0.12^{**}$ & $-0.01$      & $-0.01$      \\
                    & $(0.04)$     & $(0.03)$     & $(0.04)$     \\
\hline
R$^2$               & $0.00$       & $0.00$       & $0.00$       \\
Adj. R$^2$          & $0.00$       & $-0.00$      & $-0.00$      \\
Num. obs.           & $1791$       & $1791$       & $1791$       \\
\hline
\multicolumn{4}{l}{\scriptsize{$^{***}p<0.001$; $^{**}p<0.01$; $^{*}p<0.05$}}
\end{tabular}



==> tables/sf1989_earthquake_rank_change.tex <==

\begin{tabular}{l c c c}
\hline
 & $\Delta$ Rank 1990--1980 & $\Delta$ Rank 2000--1990 & $\Delta$ Rank 2010--2000 \\
\hline
(Intercept)         & $7.81$       & $-1.26$   & $1.86$    \\
                    & $(7.64)$     & $(6.61)$  & $(9.20)$  \\
share\_liquefaction & $-35.90^{*}$ & $5.81$    & $-8.57$   \\
                    & $(18.01)$    & $(15.59)$ & $(21.69)$ \\
\hline
R$^2$               & $0.00$       & $0.00$    & $0.00$    \\
Adj. R$^2$          & $0.00$       & $-0.00$   & $-0.00$   \\
Num. obs.           & $1791$       & $1791$    & $1791$    \\
\hline
\multicolumn{4}{l}{\scriptsize{$^{***}p<0.001$; $^{**}p<0.01$; $^{*}p<0.05$}}
\end{tabular}


